Mining Error Templates for Grammatical Error Correction

Some grammatical error correction (GEC) systems incorporate hand-crafted rules and achieve positive results. However, manually defining rules is time-consuming and laborious. In view of this, we propose a method to mine error templates for GEC automatically. An error template is a regular expression aiming at identifying text errors. We use the web crawler to acquire such error templates from the Internet. For each template, we further select the corresponding corrective action by using the language model perplexity as a criterion. We have accumulated 1,119 error templates for Chinese GEC based on this method. Experimental results on the newly proposed CTC-2021 Chinese GEC benchmark show that combing our error templates can effectively improve the performance of a strong GEC system, especially on two error types with very little training data. Our error templates are available at \url{https://github.com/HillZhang1999/gec_error_template}.

==> chapters/bak/abstract.tex <==
\begin{abstract}
Beyond spelling and grammatical errors, there is another kind of Chinese textual error called semantic errors, such as semantic duplicates and mixed syntax patterns. It is much more challenging for current automatic text proofreading systems to correct semantic errors, since their corrections usually need extensive semantic knowledge and there is no available training data yet. Therefore, most existing work handles such errors by hand-crafted rules. In this work, we propose to correct Chinese semantic errors with automatically extracted semantic templates, which reduces the heavy burden of manually defining rules. 
Concretely, we collect semantic templates from the Internet by using a web crawler and derive their corrective actions based on the perplexity from language models. Experimental results on the recently proposed CTC-2021 benchmark show that our method significantly improves the system performance to correct semantic errors. 
% such as semantic 
\end{abstract}

==> chapters/bak/introduction.tex <==
\section{Introduction}
Chinese textual error correction (CTEC) is a task aiming at detecting and correcting all underlying errors in a Chinese sentence, including spelling, grammatical and semantic errors. Compared with the other two kinds of errors, semantic errors are usually much more complex and thus are under-explored \citep{sun2022improving}. However, solving semantic errors is indispensable for the practical application of text proofreading systems due to the considerable proportion of such errors.

Previous studies on CTEC mainly focus on spelling errors \citep{wu2013chinese,yu2014overview,tseng2015introduction} and grammatical errors \citep{zhao2018overview,rao2020overview,wang2021yaclc,zhang2022mucgec}. Unlike them, semantic errors are always related to semantic information like word meanings and syntactic structures. CTC-2021 \footnote{\url{https://github.com/destwang/CTC2021}} is the first CTEC benchmark which takes semantic errors into account. CTC-2021 introduces two kinds of semantic errors, namely semantic duplicates and mixed syntax patterns. Table \ref{tab:example} shows the examples of both error types. Semantic duplicates mean that multiple components in a sentence represent the same meaning, e.g., ``大约'' (about) and ``左右'' (or so) in the first example. The mixed syntax patterns refer to the sentence phenomenon in which different syntactic structures are mixed in an expression, such as ``的起因'' (the cause of) and ``因为'' (because) in the second example. Both errors can be handled by straightforwardly deleting some sentence components.

\input{tables/examples}

Different from spelling and grammatical errors, which basically rely on deep learning models to solve now \citep{bao2020chunk,wang2021comprehensive}, existing research on recognizing and correcting Chinese semantic errors mainly adopts rule-based methods \citep{wu2015research, zhang2016study}, probably due to the lack of large-scale training data. The well-defined rules formulated by experts can effectively solve semantic errors but inevitably bring a large amount of human labor. To reduce the cost, some recent studies try to use knowledge-bases like HowNet \citep{dong2003hownet} to generate such rules \cite{zhang2021research}.

This paper proposes a simple yet effective Chinese semantic error correction method based on automatically derived semantic templates (ST). Our method only requires minimal human intervention. The basic idea is utilizing web crawlers to collect candidate semantic templates from the Internet and resort to language models to obtain corresponding corrective actions. The semantic template is a regular expression in the form of ``A.*B'', such as ``大约.*左右'' (about .* or so) in Table \ref{tab:example}. We define three kinds of corrective actions for different templates: deleting the left part (i.e., ``大约''), deleting the right part (i.e., ``左右''), and randomly selecting one part to delete. To choose an appropriate correction method for each semantic template, we adopt the perplexity calculated by language models like GPT-2 \citep{radford2019language} as a selection criteria. 

So far, we have accumulated 1,119 high-quality semantic templates using our proposed method. Experimental results on the CTC-2021 benchmark show that incorporating our semantic templates can improve the recall values from 9.59 and 7.41 to 63.01 and 40.74 for semantic duplicates and mixed syntax patterns errors, and leads to a 4.50 F${_1}$ improvement over the strong baseline, which clearly confirms the effectiveness of our method.






==> chapters/related-work.tex <==
\section{Related Work}
There has been a lot of work on Chinese spelling and grammatical error correction, including data construction \citep{tseng2015introduction, zhao2018overview, zhang2022mucgec}, model designing \citep{liu2021plome,DBLP:conf/acl/Li020} and other performance-boosting techniques like model ensembling \citep{hinson2020heterogeneous} and data augmentation \citep{zhao2020maskgec, sun2022improving}. However, little attention has been paid to semantic errors so far, which are closely related to complex semantic knowledge and thus are much more complicated.

Existing research on Chinese semantic errors primarily focuses on detection instead of correction. Some studies try to recognize semantic errors with rules defined by linguists \citep{wu2015research} or derived from semantic knowledge-bases \citep{zhang2016study,zhang2021research}. Recently, \citet{sun2022improving} argue that syntactic knowledge is crucial for recognizing semantic errors, so they design several syntax-related pre-training tasks to enhance existing pre-trained language models like BERT \citep{devlin2019bert} and utilize them to recognize semantic errors. Compared with the above-mentioned works, our work goes further into correcting semantic errors. Although our work is still based on rules, our semantic templates are automatically mined and thus avoid the cumbersome manual definition process.

